Optimization and Optimizers for Adversarial Robustness

Empirical robustness evaluation (RE) of deep learning models against adversarial perturbations entails solving nontrivial constrained optimization problems. Existing numerical algorithms that are commonly used to solve them in practice predominantly rely on projected gradient, and mostly handle perturbations modeled by the $\ell_1$, $\ell_2$ and $\ell_\infty$ distances. In this paper, we introduce a novel algorithmic framework that blends a general-purpose constrained-optimization solver PyGRANSO with Constraint Folding (PWCF), which can add more reliability and generality to the state-of-the-art RE packages, e.g., AutoAttack. Regarding reliability, PWCF provides solutions with stationarity measures and feasibility tests to assess the solution quality. For generality, PWCF can handle perturbation models that are typically inaccessible to the existing projected gradient methods; the main requirement is the distance metric to be almost everywhere differentiable. Taking advantage of PWCF and other existing numerical algorithms, we further explore the distinct patterns in the solutions found for solving these optimization problems using various combinations of losses, perturbation models, and optimization algorithms. We then discuss the implications of these patterns on the current robustness evaluation and adversarial training.

==> Sections/Adv_Robustness_Not_Generalize.tex <==
\subsection{Why pattern matters}

\paragraph{Intrinsic multiple global optimizers to the max problem}
\label{Subsec: multi-maximizers}

\js{argument/numerical evidence for the existence of multiple global optimizers, and multiple patterns}
Argument: CE and Margin Loss equation suggest multiple solutions theoretically
Numeric Evidence: May try Margin Loss with Different Initialization on a single Image.

\paragraph{Neural networks are robust to similar patterns seen during training}
\js{same norm, different patterns: any violation of the existing generalization theory? } 
Experiment: Use Lp(e.g, p=1, 4, 8, inf) attack L2 pretrained model.

==> Sections/App_Aux_Proofs.tex <==
\section{Auxiliary results and proofs} 
\label{sec:app_proofs} 



==> Sections/App_Diff_Patterns.tex <==
\section{More results on patterns induced by $\ell$, $d$, and solver}
\label{sec:app_more_patterns}

\input{Sections/section_elements/Fig-Min-Patter}

==> Sections/App_MinMax.tex <==
\section{MinMax Training for Patterns} 
\label{sec:min max} 

\input{Sections/section_elements/Table-Pattern-Compare}
% It is widely known that robustness does not generalize across even simple $\ell_p$ distance models ~\cite{maini2020adversarial,CroceHein2019Provable}. For example, $\ell_1$ distance seems to be a strong attack model for other distances such as $\ell_2$ and $\ell_\infty$, and even on itself. The patterns we discuss here provide a plausible explanation for why it is expected. Instead of digging deeper into the generalization aspect, here we focus on building reliable RE schemes, especially those non-adaptive ones that provide basic RE in the line of \texttt{AutoAttack}. In \cref{tab: pattern comare}, we quantify how different variants of loss+norm+solver+initialization+iteration combination can complement each other in terms of producing better attacks, and the message is clear: there is almost always room to complement any attack method, sometimes substantially. For example, while M+APGD seems a clear winner over our PWCF on the $\ell_1$ model, the opposite is true for the $\ell_2$ model. There never seems to be a clear winner. This reinforces the guidance on RE in~\cite{CarliniEtAl2019Evaluating,CroceEtAl2020RobustBench}: diversity of solutions matters! Meanwhile, this also highlights the fundamental difficulty of performing reliable RE: the existence of potentially infinite global maximizers with distinct patterns for \cref{eq:robust_loss} may bring back the curse of dimensionality that we try to avoid via maximization. 

==> Sections/App_Pygranso_Knitro.tex <==
\section{Comparison of \pygranso\, and \texttt{Knitro}} 
\label{sec:pygranso_knitro}

In this section, we present a comparison of \granso and \knitro on solving \cref{eq:robust_loss} with margin loss. The maximum number of iterations of both solvers is set to be 200. For \pygranso, we use 20 as limited memory size to enable limited-memory BFGS updating. For \knitro, the auto-differentiation of \texttt{PyTorch} is incorporated to make it have access to both values and gradients of the objective function and constraints through callback functions. Both solvers are initialized by the original image with a small random noise. All other parameters of the two solvers are as default.

We randomly choose 200 images from the validation set of ImageNet100 or testing set of CIFAR10 and then attack those images with \granso and \knitro. The results are shown in \cref{tab: granso_vs_knitro}. Compared to \knitro, \granso usually gets solutions with lower violation while having similar quality. And the attack success rate of \granso is higher than \knitro in most cases.

\input{Sections/section_elements/Table-Granso-vs-Knitro.tex}

==> Sections/check_list.tex <==
\section*{Checklist}


%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{}
        \item Did you include complete proofs of all theoretical results?
    \answerYes{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerNo{Code will be released after cleaning up.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerNA{Our work does not focus on model training.}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNA{}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerNA{}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{We also provide direct link to the credit the original resource in addition to cite every creator. We also explicit mention from what and how we made changes.}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{All material we used are public.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}


==> Sections/section_elements/Fig3-Sec3-Ablation-PWCF-Min-TerminateIter.tex <==
\begin{figure*}[!htbp]
\centering
\begingroup 
\setlength{\tabcolsep}{1pt}
\renewcommand{\arraystretch}{0.8}
\begin{tabular}{c c c c c c}
\centering
{}
&\multicolumn{2}{c}{\textbf{CIFAR-10}}
&{ }
&\multicolumn{2}{c}{\textbf{ImageNet}}
\\
\cline{2-3}\cline{5-6}
\vspace{-1em}
\\
{}
&\includegraphics[width=0.24\textwidth]{Figures/Sec3-Ablations/Reliability-TerminateIter/PWCF-Min-L2-Cifar.png}
&\includegraphics[width=0.24\textwidth]{Figures/Sec3-Ablations/Reliability-TerminateIter/PWCF-Min-Linf-Cifar.png}
&{ }
&\includegraphics[width=0.24\textwidth]{Figures/Sec3-Ablations/Reliability-TerminateIter/PWCF-Min-L2-ImageNet.png}
&\includegraphics[width=0.24\textwidth]{Figures/Sec3-Ablations/Reliability-TerminateIter/PWCF-Min-Linf-ImageNet.png}
\\
{}
&\small{(a) PWCF - $\ell_2$} 
&\small{(b) PWCF - $\ell_\infty$}
&{ }
&\small{(c) PWCF - $\ell_2$} 
&\small{(d) PWCF - $\ell_\infty$}

\end{tabular}
\endgroup 
\caption{Histogram of iterations where PWCF terminates in solving \formulation (\ref{eq:min_distort}). We set a maximal termination iteration $4000$ in this test.} 
\label{Fig: PWC-Min-Terminate-Iter}
\end{figure*}

==> Sections/section_elements/Table-Lp.tex <==
\begin{table}[!htpb]
\centering 
\caption{\textbf{Attack performance of PWCF with margin loss on general $\ell_p$ and non-$\ell_p$ metrics}. We report attack success rates (numbers are in $\%$). We test on $\ell_{1.5}$, $\ell_{8}$, and PAT; numbers on $\ell_1$, $\ell_2$, and $\ell_\infty$ are included for reference. Numbers below each rate in parenthesis are the perturbation radii.  }
\label{tab: granso_lp_norm}
\setlength{\tabcolsep}{1.0mm}{
%\renewcommand\arraystretch{1.25}
\begin{tabular}{l c c c c c c c}
{}
&\multicolumn{3}{c}{\small{\textbf{Special $\ell_p$}}}
&{}
&\multicolumn{3}{c}{\small{\textbf{General $\ell_p$}}}
\\
\cline{2-4}\cline{6-8}
\vspace{-8pt}
\\
\small{\textbf{Model}}
&\small{$\ell_1$}
&\small{$\ell_2$}
&\small{$\ell_\infty$}
&{}
&\small{$\ell_{1.5}$}
&\small{$\ell_8$}
&\small{PAT}
\\
% \midrule
%\hline
\toprule
%\hline
\small{Clean}
&{$100$}
&{$100$}
&{\textcolor{red}{$100$}}
&{}
&{$100$}
&{$100$}
&{$100$}
\\

&{{\footnotesize $(2361)$}}
&{{\footnotesize $(6.09)$}}
&{{\footnotesize $(0.01569)$}}
&{}
&{{\footnotesize $(44.40)$}}
&{{\footnotesize $(0.07)$}}
&{{\footnotesize $(0.5)$}}
\\
\small{PAT}
&{$49.7$}
&{$40.7$}
% &{$59.2$}
&{\textcolor{red}{$35.2$}}
&{}
&{$100$}
&{$100$}
&{$100$}
\\

&{{\footnotesize $(2400)$}}
&{{\footnotesize $(4.7)$}}
&{{\footnotesize $(0.017)$}}
&{}
&{{\footnotesize $(443.98)$}}
&{{\footnotesize $(0.70)$}}
&{{\footnotesize $(0.5)$}}
\\
\bottomrule
\end{tabular}
}
\end{table}


==> Sections/section_elements/Table-PAT-Orig-Select.tex <==
\begin{table}[!htpb]
\caption{Robust accuracy against various adversarial attacks reported in Table 3 from~\cite{laidlaw2021perceptual}. PAT-AlexNet is an adversarially trained model with the LPIPS distance. The $\ell_2$ and $\ell_\infty$ attacks during evaluation are generated by solving the \emph{max-form} using the \texttt{AutoAttack} package, whose backbone is mainly APGD with cross-entropy loss. \cite{laidlaw2021perceptual} draws the conclusion that PAT generalizes well to unforeseen perturbation types, whereas we think that PAT performs only similarly to a $\ell_2$ trained model and does not have better generalization.}
\label{tab: PAT Orig Result}
\begin{center}
\setlength{\tabcolsep}{1.0mm}{
%\renewcommand\arraystretch{1.25}
\begin{tabular}{l c c c c c c}
% \begin{tabular}{l c c c c c c c c c}
{ }
&{ }
&\multicolumn{5}{c}{\small{\textbf{Test Attack}} (Robust Acc.)}
\\
\cline{3-7}
\vspace{-10pt}
\\
\small{\textbf{Training}}
&{ }
&\small{\textbf{Clean}}
&\small{\textbf{$\ell_\infty$}}
&\small{\textbf{$\ell_2$}}
% &\small{\textbf{JPEG}}
% &\small{\textbf{StAdv}}
% &\small{\textbf{ReColor}}
&\small{\textbf{PPGD}}
&\small{\textbf{LPA}}
\\
% \midrule
%\hline
\toprule
%\hline
\small{\textbf{$\ell_\infty$}}
& { }
&{81.7}
&{55.7}
&{3.7}
% &{10.8}
% &{4.6}
% &{37.5}
&{1.5}
&{0.0}
\\
\small{\textbf{$\ell_2$}}
& { }
&{75.3}
&{46.1}
&{41.0}
% &{56.6}
% &{22.8}
% &{31.2}
&{22.0}
&{0.5}
\\
\midrule
\small{\textbf{PAT-AlexNet}}
& { }
&{75.7}
&{46.8}
&{41.0}
% &{55.9}
% &{39.0}
% &{40.8}
&{31.1}
&{1.6}
\\
\bottomrule
\end{tabular}
}
\end{center}
\end{table}


==> Sections/section_elements/Table-Sec3-Ablation-PWCF-Time.tex <==
\begin{table}[!htpb]
\caption{Statistical summary of \cref{Fig: PWC-Terminate-Time}.}
\label{tab: PWCF Time}
\begin{center}
\setlength{\tabcolsep}{1.0mm}{
\begin{tabular}{c c c c c}
\small{\textbf{Time (s)}}
&{ }
&\small{\textbf{Min}}
&\small{\textbf{Max}}
&\small{\textbf{Median}}
\\
\toprule
\small{\textbf{(a)}}
&{ }
&{0.269}
&{50.02}
&{12.37}
\\
\small{\textbf{(b)}}
&{ }
&{0.253}
&{93.62}
&{17.60}
\\
\small{\textbf{(c)}}
&{ }
&{0.377}
&{193.2}
&{36.26}
\\
\small{\textbf{(d)}}
&{ }
&{1.081}
&{131.9}
&{115.5}
\\
\midrule
\small{\textbf{(e)}}
&{ }
&{5.778}
&{134.5}
&{21.58}
\\
\small{\textbf{(f)}}
&{ }
&{91.67}
&{369.2}
&{167.5}
\\
\small{\textbf{(g)}}
&{ }
&{2.965}
&{354.8}
&{112.9}
\\
\small{\textbf{(h)}}
&{ }
&{121.5}
&{317.0}
&{161.7}
\\
\bottomrule
\end{tabular}
}
\end{center}
\end{table}


==> sn-sample-bib.tex <==
\begin{thebibliography}{9}

\bibitem{bib1} I.~Podlubny, Fractional Differential Equations, Academie Press, New York, 1999.

\bibitem{bib2} R. Hilfer, Application of Fractional Calculus in Physics, World Science Publishing, Singapore, 2000.

\bibitem{bib3} A. Nagih, G. Plateau, Fractional problems: overview of applications and solutions. Rairo-Recherche Operationnelle-Oper Press, New York, 1999.

\bibitem{bib4} J. P. Richard, Time-delay system: an overview of some recent advances and open problems, Automatica, 39(10) (2003) 1667-1694.

\bibitem{bib5} H. Ye, J. Gao, Y. Ding, A generalized Gronwall inequality and its application to a fractional differential equation, J. Math. Anal. Appl., 328 (2007) 1075-1081.

\bibitem{bib6} M. Lazarevic, Stability and stabilization of fractional order time delay systems, Scientific Technical Review, 61 (2011) 31-45.

\bibitem{bib7} Y. Li, Y. Q. Chen, I. Podlubny, Stability of fractional-order nonlinear dynamic systems: Lyapunov direct method and generalized Mittag-Leffler stability, Comp. Math. Appl., 59 (2010) 1810-1821.


\end{thebibliography}


